Balancing Constraints and Rewards with Meta-Gradient D4PG

Deploying Reinforcement Learning (RL) agents to solve real-world applications often requires satisfying complex system constraints. Often the constraint thresholds are incorrectly set due to the complex nature of a system or the inability to verify the thresholds offline (e.g, no simulator or reasonable offline evaluation procedure exists). This results in solutions where a task cannot be solved without violating the constraints. However, in many real-world cases, constraint violations are undesirable yet they are not catastrophic, motivating the need for soft-constrained RL approaches. We present a soft-constrained RL approach that utilizes meta-gradients to find a good trade-off between expected return and minimizing constraint violations. We demonstrate the effectiveness of this approach by showing that it consistently outperforms the baselines across four different MuJoCo domains.

==> defs.tex <==
\newcommand{\cp}{\citep}
\newcommand{\ca}{\citeauthor}
\newcommand{\cy}{\citeyear}
\newcommand{\ct}{\citet}
\newcommand{\ctp}[1]{\ca{#1}'s~(\cy{#1})}
\newcommand{\cwp}[1]{\ca{#1}, \cy{#1}}
\newcommand{\ctt}[1]{\ca{#1}~\cp{#1}} %

\newcommand{\mat}[1]{\ensuremath{\boldsymbol{\mathrm{#1}}}}
\newcommand{\fnc}[1]{\ensuremath{\mathrm{#1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}

\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\M}{\ensuremath{\mathcal{M}^{\phi}}}
\newcommand{\MM}{\ensuremath{\mathcal{M}}} 
\newcommand{\CC}{\ensuremath{\mathcal{C}}} 
\newcommand{\E}{\ensuremath{\mathrm{E}}}
\newcommand{\MMtr}{\ensuremath{\hat{\MM}}} 
\newcommand{\Mtr}{\ensuremath{\hat{M}}}
\newcommand{\wtr}{\ensuremath{\hat{\mat{w}}}}
\newcommand{\rtr}{\ensuremath{\hat{r}}}
\newcommand{\rvtr}{\ensuremath{\hat{\mat{r}}}}
\newcommand{\Rtr}{\ensuremath{\hat{R}}}
\newcommand{\Wtr}{\ensuremath{\hat{\mat{W}}}}

\newcommand{\Normal}{\ensuremath{\mathcal{N}}}

\newcommand{\w}{\mat{w}}
\newcommand{\WW}{\mat{W}}
\newcommand{\Wt}{\ensuremath{\tilde{\mat{W}}}}
\renewcommand{\r}{\mat{r}}
\newcommand{\z}{\mat{z}}
\newcommand{\zw}{\mat{zw}}
\newcommand{\Z}{\mat{Z}}
\newcommand{\vphi}{\mat{\phi}}
\newcommand{\vpsi}{\mat{\psi}}
\newcommand{\vprm}{\mat{\z}}
\newcommand{\tvphi}{\ensuremath{\tilde{\mat{\phi}}}}
\newcommand{\tvpsi}{\ensuremath{\tilde{\mat{\psi}} }}
\newcommand{\tPsi}{\ensuremath{\tilde{\Psi} }}
\newcommand{\tmpsi}{\ensuremath{\tilde{\mat{\Psi}} }}
\newcommand{\MPhi}{\mat{\Phi}}
\newcommand{\MPsi}{\mat{\Psi}}
\renewcommand{\P}{\mat{P}}
\renewcommand{\t}{\ensuremath{\top}}



\renewcommand{\th}[1]{\text{#1$^\mathrm{th}$}}
\newcommand{\ith}{\th{i}}
\newcommand{\jth}{\th{j}}
\newcommand{\kth}{\th{k}}

\newcommand{\argmin}{\ensuremath{\mathrm{argmin}}}
\newcommand{\argmax}{\ensuremath{\mathrm{argmax}}}
\renewcommand{\min}{\ensuremath{\mathrm{min}}}

\newcommand{\Qmax}{\ensuremath{Q_{\mathrm{max}}}}
\newcommand{\pimax}{\ensuremath{\pi_{\max}}}
\newcommand{\Qpimax}{\ensuremath{Q^{\pi_{\max}}}}
\newcommand{\Tpimax}{\ensuremath{T^{\pi_{\max}}}}

\newcommand{\Mh}{\ensuremath{\hat{M}}} 
\newcommand{\Qh}{\ensuremath{\hat{Q}}}
\newcommand{\pih}{\ensuremath{\hat{\pi}}}
\newcommand{\wh}{\ensuremath{\hat{\w}}}
\newcommand{\Qhmax}{\ensuremath{\hat{Q}_{\mathrm{max}}}}
\newcommand{\pihmax}{\ensuremath{\pi}}
\newcommand{\Qhpimax}{\ensuremath{\hat{Q}^{\pi_{\max}}}}
\newcommand{\Thpimax}{\ensuremath{\hat{T}^{\pi_{\max}}}}

\newcommand{\rdif}{\ensuremath{\delta}}

\newcommand{\Qt}{\ensuremath{\tilde{Q}}}
\newcommand{\vQt}{\ensuremath{\tilde{\mat{Q}}}}
\newcommand{\pit}{\ensuremath{\tilde{\pi}}}
\newcommand{\Qtmax}{\ensuremath{\tilde{Q}_{\mathrm{max}}}}
\newcommand{\pitmax}{\ensuremath{{\pi}}}
\newcommand{\Qpitmax}{\ensuremath{Q^{\pi}}}
\newcommand{\Tpitmax}{\ensuremath{T^{\pi}}}
\newcommand{\wt}{\ensuremath{\tilde{\w}}}
\renewcommand{\H}{\mat{H}} 

\newcommand{\agt}{\fnc{agt}}

\newcommand{\piexp}{\ensuremath{\pi}}
\newcommand{\piexpj}{\ensuremath{_{\piexp_j}}}
\newcommand{\piexpi}{\ensuremath{_{\piexp_i}}}
\newcommand{\piexpk}{\ensuremath{_{\piexp_k}}}

\newcommand{\la}{\ensuremath{\leftarrow}}

\newcommand{\vpi}{\ensuremath{\mat{v}^{\pi}}}
\newcommand{\rpi}{\ensuremath{\mat{r}^{\pi}}}
\newcommand{\Ppi}{\ensuremath{\mat{P}^{\pi}}}

\newcommand{\phimax}{\ensuremath{\vphi_{\max}}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}

\newcommand{\score}{\ensuremath{\mathrm{score}}}
\newcommand{\currscore}{\ensuremath{\mathrm{curr\_score}}}
\newcommand{\ntpu}{\ensuremath{\mathrm{used}}}
\newcommand{\act}{\ensuremath{\mathrm{c}}}

\newcommand{\I}[1]{\ensuremath{\delta\{#1\}}} 
\newcommand{\II}{\ensuremath{\delta}} 

\newcommand{\vf}{\ensuremath{\mat{\varphi}}}
\newcommand{\vfi}{\ensuremath{\mat{\varphi}_i}}
\newcommand{\vfp}{\ensuremath{\mat{\varphi}_p}}
\newcommand{\vweights}{\mat{z}}
\newcommand{\od}{\ensuremath{\mat{o}}}
\newcommand{\rank}{\ensuremath{\mathrm{rank}}}

\newcommand{\ns}{\ensuremath{\mathrm{ns}}}
\newcommand{\nstr}{\ensuremath{n_{\mathrm{tr}}}}
\newcommand{\nsts}{\ensuremath{n_{\mathrm{ts}}}}
\newcommand{\dist}{\ensuremath{\mathcal{D}}}
\newcommand{\rt}{\ensuremath{\tilde{r}}}
\newcommand{\rvt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\vrt}{\ensuremath{\tilde{\mat{r}}}}
\newcommand{\params}{\ensuremath{\mat{\theta}}}

\newcommand{\eb}{\ensuremath{\mathrm{extend\_basis}}}
\newcommand{\sfgpi}{SF\hspace{0.2mm}\&\hspace{0.2mm}GPI}
\newcommand{\sfgpirl}{\sfgpi\ continual}
\newcommand{\sfgpisl}{\sfgpi\ zero-shot}

\newcommand{\mo}{{\normalfont-{\tt 1}}}
\newcommand{\taskfive}{{\tt 1100}}
\newcommand{\tasksix}{{\tt 0111}}
\newcommand{\taskseven}{{\tt 1111}}
\newcommand{\taskeight}{{\tt \mo000}}
\newcommand{\tasknine}{{\tt \mo\mo00}}
\newcommand{\taskten}{{\tt \mo100}}
\newcommand{\taskeleven}{{\tt \mo1\mo0}}
\newcommand{\tasktwelve}{{\tt \mo101}}
\newcommand{\taskthirteen}{{\tt \mo1\mo1}}
\newcommand{\taskexample}{{\tt 1\mo00}}


\newcommand{\pitest}{\ensuremath{\pi_{\mathrm{test}}}}

\renewcommand{\dist}{\ensuremath{\mathcal{D}}}

\newcommand{\tderrorz}{\ensuremath{\mat{\delta}_{\z}^{t,n}}}
\newcommand{\tderrorwz}{\ensuremath{\mat{\delta}_{\w\z}^{t,n}}}
\newcommand{\deriv}{\mathrm{d}}
